VISPUR: Visual Aids for Identifying and Interpreting Spurious Associations in Data-Driven Decisions

Big data and machine learning tools have jointly empowered humans in making data-driven decisions. However, many of them capture empirical associations that might be spurious due to confounding factors and subgroup heterogeneity. The famous Simpson's paradox is such a phenomenon where aggregated and subgroup-level associations contradict with each other, causing cognitive confusions and difficulty in making adequate interpretations and decisions. Existing tools provide little insights for humans to locate, reason about, and prevent pitfalls of spurious association in practice. We propose VISPUR, a visual analytic system that provides a causal analysis framework and a human-centric workflow for tackling spurious associations. These include a CONFOUNDER DASHBOARD, which can automatically identify possible confounding factors, and a SUBGROUP VIEWER, which allows for the visualization and comparison of diverse subgroup patterns that likely or potentially result in a misinterpretation of causality. Additionally, we propose a REASONING STORYBOARD, which uses a flow-based approach to illustrate paradoxical phenomena, as well as an interactive DECISION DIAGNOSIS panel that helps ensure accountable decision-making. Through an expert interview and a controlled user experiment, our qualitative and quantitative results demonstrate that the proposed "de-paradox" workflow and the designed visual analytic system are effective in helping human users to identify and understand spurious associations, as well as to make accountable causal decisions.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> images/Acc_v2_caption.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/Acc_v2.pdf}
    \caption{Mean and confidence interval (obtained from R = 999 bootstrap samples) for the overall accuracy (A) as well as the question-specific accuracy (B). Bar chart indicates mean, error bar means CI, $p-$values are obtained from the associated paired Wilcoxon signed-rank test comparing \vispur and baseline.}
    \label{fig:accuracy}
\end{figure}

==> images/Certainty_v2_caption.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/Certainty_v2.pdf}
    \caption{Mean and confidence interval (obtained from R = 999 bootstrap samples) for the overall certainty (A) as well as the question-specific certainty (B). Bar chart indicates mean, error bar means CI, $p-$values are obtained from the associated paired Wilcoxon signed-rank test comparing \vispur and baseline.}
    \label{fig:certainty}
\end{figure}



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/700_discussion.tex <==
\section{Discussion}\label{sec:discussion}

{We discuss the usability of \vispur system, common human behaviors in using it, and the limitations as well as future directions.}

{\bf Usability of \vispur's components.} Study participants and experts provided positive feedback on the usability and effectiveness of \vispur. We especially found that The \confounderdashboard and \subgroupviewer (along with \partition) components were heavily used by human users to examine distortion effect from confounders and the mixed effect from subgroups. As commented by a subject: ``{\it \vispur let me know more information about subgroups than baseline.}'' When asked to explain Simpson's paradox, four participants mentioned that \vispur's flow charts in \reasoningstoryboard were more intuitive than baseline, as it ``clearly shows data splits'' and ``how data flows through cause to outcome.'' Besides, many users reported that it reminded them of overlooked information and prevented them from making imprudent decisions. The warning messages and imbalance chart features in \decisiondiagnosis were praised by participants and experts for triggering further thinking and helping to locate residual confounders. Additionally, \vispur was found to be useful in generating and validating hypotheses, as well as delivering analysis results to decision-makers or colleagues. As Micheal commented, ``{\it I do not need to plot and explain a lots of figures by myself, I can just modify partitions and discuss the visualizations produced by \vispur with my boss.}''

{\bf Human behaviors in paradox reasoning and decision-making.} Although \vispur improved participants' answering accuracy, questions related to paradox reasoning and decision-making still posed a challenge. When asked to agree or disagree with an explanation for paradoxical associations, many participants struggled to connect observed visual evidence to a final statement. Additionally, many participants relied on their subjective tendency when making a decision, rather than utilizing the system. For instance, one participant stated that they recommended a person take a training program because ``{\it taking a training shouldn't be bad},'' regardless of \vispur's visualizations. To aid such challenging cognitive tasks, a possible solution in the future could be to support interactive collaborations on a visual analytic system among users. For instance, users can highlight visualizations, leave their interpretations, and share ideas to reach a final conclusion.
% {E.g., they could find visual evidence that was concordant or discordant to the first part of the description: {\it the old participants are more likely to take the online course while the reverse is true for the young; meanwhile, they also tend to have a higher likelihood of passing the exam than the young}, however, they made mistakes whilst connecting such visual evidence to the final statement: {\it these two factors---``those who likely to take the treatment happen to be those who likely to succeed''---result in a spurious positive association overall}.}


{\bf Limitation and future work.} We summarize the limitation and the possible future work to tackle those issues.

\begin{enumerate}
    \item \tocomments{\bf Mental causal model and violation of causal framework.} {Although \vispur offers qualitative scores and visual signals to identify confounders, it is important to note that human beliefs and assumptions about causal structure are still necessary. Relying solely on statistical criteria can lead to adjusting for undesirable variables if there is insufficient causal knowledge about the sources of confounding \cite{hernan2020causal}. To mitigate this issue, the use of causal DAG has been suggested and implemented in many causal reasoning tools \cite{yen2019exploratory}. These DAGs capture users' mental models of how variables are related and facilitate reflection on common causes of treatment and outcome as a sufficient set of adjustment variables. In future work, \vispur could be expanded to include a DAG panel that allows users to draw DAGs before exploring confounding tendency scores and visual information. This would encourage causal reflection and explicitly incorporate domain knowledge.}
    
    \item {\bf Scalability.} \vispur is capable of generating subgroups using an unlimited list of partition rules or by utilizing machine learning algorithms to search for optimal partitions. However, the system has limited scalability when dealing with a large number of subgroups. In such cases, the \causalityspace may become crowded, making it difficult to visually distinguish between different subgroups. Future work could address this issue by introducing flexible subgroup operations, such as hierarchical subgrouping, filtering, hiding, highlighting, and zooming in/out, to mitigate issues such as overlapping visualizations and information overload. These operations would allow for effective exploration and comparison of subgroups, ultimately improving the usefulness of the system.
    \item {\bf Imbalance representation.} The \imbalancechart in \decisiondiagnosis (ref. Section~\ref{sec:systemdesign:decisiondiagnosis}) effectively identifies variables with high imbalance scores. However, users with limited knowledge of causality may struggle to grasp the concept of imbalance. Future work could focus on designing an intuitive visual representation to enhance users' understanding, such as visualizing the association between pretreatment variables and treatment, or showcasing the distributions of pretreatment variables across treatment arms.
\end{enumerate}

% {{\bf System guidelines.} \ysc{Shall we remove this part?} Participants in our study session had the chance of getting familiar with \vispur by watching a tutorial video, followed by a self-exploration practice, but a desire for embedded guidelines was a consistent theme to make the system more self-contained and independent from external training. We observed that, participants might forget the meanings of certain visual encodings (e.g., size of circles, axes of radar charts etc), or had no idea what actions (e.g., click, select) to perform to retrieve useful information. Without appropriate guidelines, some participants got confused regarding the variables used in different places, such as in confounder table, in radar charts, and in imbalance chart. A participant commented: ``{\it I hope the system could automatically remind me where to click and what next step to take.} A participant expressed the desire for a new functionality that users could generate analysis reports for teamwork communication and result delivery.}
